LHCb VELO Timepix3 Telescope

The LHCb VELO Timepix3 telescope is a silicon pixel tracking system constructed initially to evaluate the performance of LHCb VELO Upgrade prototypes. The telesope consists of eight hybrid pixel silicon sensor planes equipped with the Timepix3 ASIC. The planes provide excellent charge measurement, timestamping and spatial resolution and the system can function at high track rates. This paper describes the construction of the telescope and its data acquisition system and offline reconstruction software. A timing resolution of 350~ps was obtained for reconstructed tracks. A pointing resolution of better than 2~\mum was determined for the 180~GeV/c %\gevc mixed hadron beam at the CERN SPS. The telescope has been shown to operate at a rate of 5 million particles~\unit{s^{-1}\cdot cm^{-2}} without a loss in efficiency.

==> online.tex <==
\subsection{Online Monitoring}\label{online}
%\begin{itemize}
%\item{description of its goals}
%\item{software used, C++, QT etc., separate DAQ stream}
%\item{structure, hierarchy, plots produced }
%\item{example plots}
%\end{itemize}

%A small dedicated software framework has been developed for online Data Quality Monitoring (DQM) of the 
%telescope. This software reconstructs clusters and tracks from the raw data stored on the DAQ
%computer and  verifies the acquired data is of good quality.% Data are read from the raw files stored on the DAQ computers.

A small dedicated software framework has been developed for online Data Quality and 
Monitoring (DQM) of the telescope. This package uses simple and robust algorithms to 
reconstruct clusters and tracks from the raw data and to ensure the acquired data is of 
good quality for DUT studies. The DQM package obtains its data by reading the raw 
data from files stored on the DAQ computers.


%This package uses simple and robust algorithms to reconstruct clusters and tracks from the raw data
%and ensures the acquired data is of good quality for DUT studies.
%The DQM package obtains its data by reading the raw data from files stored on the DAQ computers.
%\footnote{Alternatively, the Timepix3 DAQ is able to provide a fraction of the full data sample as a separate data stream, via
%ethernet, at set intervals (monitoring stream).
%The DQM could use this reduced stream to spy and process the acquired data online, when running at high rates.}.

%The DQM main purpose is for: 
%\begin{itemize}
%\item Checking telescope alignment with particle beam;
%\item Ensuring telescope planes are synchronised by looking at time and spatial correlations between planes;
%\item Providing an easy way to check the spatial alignment of the Timepix3 based DUTs; 
%\end{itemize}

The online monitoring package is written as a standalone C++ application, 
using ROOT \cite{root} and Qt \cite{qt} %libraries. 
libraries for a Graphics User Interface (GUI). Quantities included in the monitoring 
are hitmaps, cluster size distributions, cluster positions, ToT distributions and hit 
correlations between planes.

%The Qt based Graphics User Interface (GUI) of the DQM package is used to visualise 
%all monitoring results, which include the hitmaps for all sensors, cluster size distributions,
%cluster positions, Landau fitted ToT distributions for both hits and clusters and hit correlations between planes. 
A screenshot of this GUI is shown in figure~\ref{fig:dqmgui}.
  \begin{figure}[!htb]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/DQMtriple.png}
    \caption{Screenshot of the visual interface for online data quality monitoring. In this instance the
GUI is displaying hit maps for the eight telescope arms (top and bottom rows) and for the DUT  (centre row), a
sensor bonded to three Timepix3 ASICs.} 
    \label{fig:dqmgui}
  \end{figure}


%In this way the telescope planes and beam related parameters can be instantaneously
%monitored, allowing easy control of the telescope for the shifter.


%The DQM will soon be able to interface with the VeloPix ASIC, allowing the DQM to also be used for DUT studies with the VeloPix ASIC.



==> trackefficiency.tex <==

\subsection{Tracking Efficiency}\label{trackeff}



The efficiency of a tracking system is defined as the fraction of charged particles passing through all 
measuring stations that are successfully reconstructed as a track.
In order to estimate the tracking efficiency it would be necessary to have a known 
number of tracks traversing the whole telescope acceptance, which is impossible without  external information.
For this reason, the fraction of associated clusters to a track is used as a figure of merit for efficiency.
%In the case where 
If all clusters in the telescope originated from tracks that entered the telescope,
this fraction would converge to the efficiency.
%However, if  a track interacts with material producing secondary tracks,
%the clusters could be generated by tracks which didn't cross all telescope planes. 
In practice, some  clusters originate from secondary charged 
particles produced in the telescope material, or from primary
particles which only pass through part of the telescope.
These secondary tracks are often angled and produced in the middle of the telescope
which makes it  difficult to reconstruct or identify all of them. 
To account for this effect an occupancy cut is defined as maximum the number of clusters in within
a time window of 10 ns of a seed cluster.  This cut is used to remove from the analysis sample 
particles that produce  spurious secondary tracks. Figure~\ref{Fig:TrackEfficiency} 
shows the fraction of associated clusters as a function of occupancy cut. 
In a typical run, with about 2 million particles per 4s spill, the fraction of associated clusters
is 98\% if exactly eight clusters were detected in the whole telescope with one cluster per plane.
 

\begin{figure}[!htb]
\centering
%\includegraphics[width=0.45\textwidth]{figs/clusterOccupancy.pdf}
\includegraphics[width=1.\textwidth]{figs/TrackingEfficiencyRootVersion_auto.png}
\caption{Fraction of associated clusters as a function of occupancy requirement.}
\label{Fig:TrackEfficiency}
\end{figure}


